Can We Trust AI-Inferred User States. A Psychometric Framework for Validating the Reliability of Users States Classification by LLMs in Operational Environments

The use of large language models to assess user states in conversational and adaptive systems is based on the assumption that the metrics used for such assessment are stable and interpretable at the level of individual scores. This paper empirically tests this assumption, focusing on the psychometric reliability of artificial intelligence (AI) measures of user states. This study employed replication evaluation procedures to assess the repeatability of a broad set of metrics across three different bimodal large language models (GPT-4o audio, Gemini 2.0 Flash, Gemini 2.5 Flash). Analyses include both individual score reliability and aggregated reliability, allowing us to distinguish metrics potentially useful for real-time adaptation from those that retain their value only in aggregated analyses. The results demonstrate that metric reliability cannot be considered a default property in interpretive domains. The lack of stability at the level of individual scores precludes the interpretation of such scores as indicators of user state in real-time adaptive systems, even if these metrics demonstrate stability after aggregation. At the same time, the study indicates that individually unstable metrics can retain analytical utility in post-hoc studies, identifying rules governing interactions and their relationships with user experience parameters such as satisfaction, trust, and engagement. The main contribution of this work, besides quantifying the severity of the problem (only 31 of 213 metrics met the criteria), is the proposal of a replicable evaluation framework, enabling measurable evaluations of metric applicability. This approach supports more responsible AI design of adaptive systems, in which the interpretation of results requires explicit validation of reliability and monitoring for violations over time.

==> agreement_tables.tex <==
\begin{table}[]
\centering
\caption{Summary of normalized median Mean Absolute Error and median Cohen's Kappa agreement levels between model pairs:  A - GPT4o vs Gemini 2.0; B - GPT4o vs Gemini 2.5; C - Gemini 2.0 vs Gemini 2.5 across 31 features that demonstrated excellent single-inference reliability (ICC(3,1) $\geq 0.9$) in all three models.  Cell values indicate count of features meeting each criterion.
}
\label{tab:study3_31}
\begin{tabular}{lllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Interpretation}}} &
  \multicolumn{4}{c}{\textbf{norm med MAE}} &
  \multicolumn{4}{c}{\textbf{med $\kappa$}} \\ \cline{2-9} 
\multicolumn{1}{c}{} &
  \textbf{range} &
  \textbf{A} &
  \textbf{B} &
  \textbf{C} &
  \textbf{range} &
  \textbf{A} &
  \textbf{B} &
  \textbf{C} \\ \hline

  \rowcolor[HTML]{90EE90}almost perfect                                               & \textless 0.05    & 19 & 9 & 9  & 0.80-1.0                      & 0 & 0 & 0 \\
  \rowcolor[HTML]{E0FFE0}substantial                                                  & 0.05-0.10                        & 4  & 6 & 5  & 0.60-0.80                     & 0 & 0 & 0 \\
  \rowcolor[HTML]{FFFFE0}moderate                                                     & 0.10-0.20                        & 2  & 7 & 10 & 0.40-0.60                     & 2 & 0 & 0 \\
  \rowcolor[HTML]{FFE0E0}poor                                                         & \textgreater 0.20 & 4  & 7 & 5  & \textless 0.4  & 0 & 2 & 2 \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{Summary of normalized median Mean Absolute Error and median Cohen's Kappa agreement levels between model pairs:  A - GPT4o vs Gemini 2.0; B - GPT4o vs Gemini 2.5; C - Gemini 2.0 vs Gemini 2.5 across 89 features that demonstrated excellent averaged-inferences reliability (ICC(3,k) $\geq 0.9$) in all three models.  Cell values indicate count of features meeting each criterion.
}
\label{tab:study3_89}
\begin{tabular}{lllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Interpretation}}} &
  \multicolumn{4}{c}{\textbf{norm med MAE}} &
  \multicolumn{4}{c}{\textbf{med $\kappa$}} \\ \cline{2-9} 
\multicolumn{1}{c}{} &
  \textbf{range} &
  \textbf{A} &
  \textbf{B} &
  \textbf{C} &
  \textbf{range} &
  \textbf{A} &
  \textbf{B} &
  \textbf{C} \\ \hline
\rowcolor[HTML]{90EE90}almost perfect  & \textless 0.05    & 34 & 22 & 28 & 0.80-1.0                     & 1 & 0 & 0 \\
\rowcolor[HTML]{E0FFE0}substantial    & 0.05-0.10                        & 20 & 21 & 16 & 0.60-0.80                    & 1 & 1 & 1 \\
\rowcolor[HTML]{FFFFE0}moderate       & 0.10-0.20                        & 6  & 4  & 5  & 0.40-0.60                    & 5 & 1 & 2 \\
\rowcolor[HTML]{FFE0E0}poor           & \textgreater 0.20 & 15 & 19 & 12 & \textless 0.4 & 0 & 5 & 4 \\ \hline
\end{tabular}
\end{table}

==> feature_prompts.tex <==

\newpage
\small
\section{AdaptiveDynamicsAnalysis}

\subsection{Actual Strategy Time}

\begin{description}
\item[Description:]
\begin{quote}
Duration of current strategy (Metric 1.1)A quantitative measure, expressed in terms of the number of consecutive conversational turns or units of time, of how long a system maintains a single, consistent communication strategy (e.g., empathetic listening, data gathering, step-by-step instruction) without changing.\par

\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'same\_strategy\_turns'}: int (number of turns Calculate based on dialogue history and strategy name)
\item \texttt{'strategy\_name'}: str (name of the actual strategy)
\end{itemize}
\end{quote}
\end{description}

\subsection{User Patterns Changing}

\begin{description}
\item[Description:]
\begin{quote}
Changing User Speech Patterns  (Metric 1.2)Analyze only customer's messages to detect shifts in their engagement and emotional state. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'last\_user\_message'}: str (last customer message) (if unable to calculate return 'N/A')
\item \texttt{'emotional\_valence'}: float (-1.0-1.0, Shift towards positive/negative sentiment, if unable to calculate return 0.0)
\item \texttt{'linguistic\_complexity'}: float (0.0-100.0,  Percent change in the number of words. If unable to calculate (first turn) return 0.0)
\end{itemize}
\end{quote}
\end{description}

\subsection{Tone Topic Fluctuations}

\begin{description}
\item[Description:]
\begin{quote}
Number of ambiguous response ratings (Metric 1.3) using formula:

$\texttt{transition\_entropy} = - \sum [P(strategy\_i) * log\_2(P(strategy\_i))]$

transition\_entropy: Entropy score for the conversation window.

P(strategy\_i): Probability of occurrence of a given strategy i in the analyzed window. Calculated as Count(strategy\_i) / TotalTurns. 

$\sum$: Sum after all unique strategies that appeared in the window.
\par

\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'transition\_entropy\_score'}: float (calculate using formula), if unable to calculate return 0.0
\item \texttt{'strategy\_distribution'}: dict\textless{}float\textgreater{} (keys: strategies names, values: distribution
\item \texttt{'assessment'}: str (clear explanation)
\end{itemize}
\end{quote}
\end{description}

\subsection{Response Accuracy Decrease}

\begin{description}
\item[Description:]
\begin{quote}
Analyzing relevance trend (Metric 1.4) 
Determine if the system's relevance is decaying based on the equation:
\texttt{relevance\_decay} = slope(linear\_regression([semantic\_relevance(t-n)...semantic\_relevance(t)]))semantic\_relevance(t) = cosine\_similarity(embedding(user\_query\_t), embedding(system\_response\_t))semantic\_relevance(t): 
Reliability in turn t, calculated e.g. as the cosine similarity between the vector representations of the query and the answer.relevance\_decay: Slope of the linear regression line fitted to the series of accuracy scores from the last n rounds.slope \textless{} 0: negative decay slope $\approx 0$: stable slope \textgreater{} 0: positive decay\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'relevance\_decay'}: float (0-1, calculate using formula)
\item \texttt{'trend'}: \textless{}Improving\textbar{}Stable\textbar{}Decaying\textgreater{} (characterize the trend)
\end{itemize}
\end{quote}
\end{description}

\subsection{Dialog Progression}

\begin{description}
\item[Description:]
\begin{quote}
Dialog stagnation calculated as:

\(\texttt{stagnation\_score} = w_{loop}  \cdot  loop\_detection\_ score + w_{info}  \cdot  new\_info\_decay\), where:

$loop\_detection\_ score$: Score (0-1) from a loop detection algorithm, calculated by comparing the semantic similarity of $user\_query_{t} $
with 
$user\_query_{t-n}$ 

and $system\_response_{t}$ with $system\_response_{t-n}$. 
High similarity in both pairs indicates a loop.

$new\_info\_decay$: A measure of the decrease in the number of new, key information units (entities) introduced to the dialogue in subsequent rounds, If no new entities have appeared in n rounds, the score is high

$w_{loop}$, $w_{info}$: Weights given to individual components
\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'stagnation\_score'}: float (0-1, calculate using formula)
\item \texttt{'findings'}: \{
\begin{itemize}
    \item \texttt{'loop\_detected'}: \textless{}true/false\textgreater{},
\item \texttt{'new\_info\_flow'}: '\textless{}High\textbar{}Medium\textbar{}Low\textbar{}None\textgreater{}'\textgreater{}),
\item \texttt{'diagnosis'}: str (short explanation what's wrong in the conversation)\}
\end{itemize}

\end{itemize}
\end{quote}
\end{description}

\subsection{Ambiguity Resolving Cost}

\begin{description}
\item[Description:]
\begin{quote}
Ambiguity costs calculated as:

$\texttt{ambiguity\_cost} = count(clarification\_turns) + max(0, count(presented\_options) - 1)$, where:

$clarification\_turns$: Number of complete dialogue turns spent asking a question and receiving a clarifying answer

$presented\_options$: The number of options presented to the client to choose from \par

\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'ambiguity\_cost'}: int (calculated using formula)
\item \texttt{'clarification\_turns'}: int (number of turns used to clarification)
\item \texttt{'is\_ambiguous\_query'}: bool (indicate if the question was ambiguous)
\end{itemize}
\end{quote}
\end{description}

\subsection{Follow Up Query Type}

\begin{description}
\item[Description:]
\begin{quote}
Follow-up Query Type calculated as:

$\texttt{fuq\_type} = classifier(system\_response, user\_follow\_up)$, where:

classifier: Classify pairs of utterances strictly into categories defined in the following taxonomy: 'Correction', 'Refinement', 'Elaboration', 'New Question (Related)', 'New Question (Unrelated)', 'N/A' (in case unable to classify) \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'fuq\_type'}: str (predict using formula)
\item \texttt{'confidence'}: float (0-1)
\end{itemize}
\end{quote}
\end{description}

\section{AffectAnalysis}

\subsection{Valence Arousal Scales}

\begin{description}
\item[Description:]
\begin{quote}
Valence and arousal assessment calculated using formulas: 

$\texttt{Valence} = va\_weights['alpha']·text\_valence + va\_weights['beta']·audio\_valence$

$\texttt{Arousal} = va\_weights['gamma']·text\_arousal + va\_weights['delta']·audio\_arousal$ 
\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'valence'}: float (calculated from formula),
\item \texttt{'arousal'}: float (calculated from formula),
\item \texttt{'text\_valence'}: float (valence derived from text analysis),
\item \texttt{'audio\_valence'}: float (valence derived from audio analysis),
\item \texttt{'text\_arousal'}: float (arousal derived from text analysis),
\item \texttt{'audio\_arousal'}: float (arousal derived from audio analysis),
\item \texttt{'emotional\_quadrant'}: str (one of: 'positive\_high\_arousal', 'positive\_low\_arousal', 'negative\_high\_arousal', 'negative\_low\_arousal'),
\item \texttt{'interpretation'}: str (explanation of emotional state and recommended consultant response).
\end{itemize}
\end{quote}
\end{description}

\subsection{Prosodic Features}

\begin{description}
\item[Description:]
\begin{quote}
Prosodic feature extraction from voice using formula: \texttt{EmotionalState} = \(w_1 \cdot F0Norm + w_2 \cdot TempoNorm + w_3 \cdot IntensityNorm + w_4 \cdot JitterNorm + w_5 \cdot HNRNorm\). \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'pitch\_statistics'}: \{
\begin{itemize}
    \item \texttt{'mean'}: float (Hz),
    \item \texttt{'std'}: float (Hz),
    \item \texttt{'min'}: float (Hz),
    \item \texttt{'max'}: float (Hz),
    \item \texttt{'range'}: float (Hz)\},
\end{itemize}
\item \texttt{'tempo\_speaking'}: float (syllables per second),
\item \texttt{'intensity\_rms'}: float (RMS intensity),
\item \texttt{'zero\_crossing\_rate'}: float (ZCR),
\item \texttt{'jitter'}: float (voice irregularities as ratio),
\item \texttt{'hnr'}: float (Harmonics-to-Noise Ratio in dB),
\item \texttt{'pause\_patterns'}: \{
\begin{itemize}
    \item \texttt{'count'}: int,
    \item \texttt{'average\_duration'}: float (seconds),
    \item \texttt{'total\_duration'}: float (seconds)\},
    \item \texttt{'normalized\_features'}: \{'f0\_norm': float (0-1),
    \item \texttt{'tempo\_norm'}: float (0-1),
    \item \texttt{'intensity\_norm'}: float (0-1),
    \item \texttt{'jitter\_norm'}: float (0-1),
    \item \texttt{'hnr\_norm'}: float (0-1)\},
\end{itemize}

\item \texttt{'feature\_weights'}: \{'w1': float, 'w2': float, 'w3': float, 'w4': float, 'w5': float\} (summing to 1.0),
\item \texttt{'emotional\_state\_score'}: float (0-1, calculated from prosodic features using formula),
\item \texttt{'stress\_indicators'}: list (identified stress markers in voice),
\item \texttt{'voice\_quality\_assessment'}: str (overall voice quality description)
\end{itemize}
\end{quote}
\end{description}

\subsection{Semantic Content Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Semantic content analysis for emotional identification using formula: 

$\texttt{BaseSentiment} = (PosWords - NegWords) / TotalWords$

$\texttt{IntensityMultiplier} = 1 + AbsolutismFactor \cdot AbsWords/TotalWords$

$\texttt{SentimentScore} = clamp(BaseSentiment \cdot IntensityMultiplier, -1.0, 1.0).$ 
\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'emotional\_words'}: \{
\begin{itemize}
    \item \texttt{'positive'}: list,
    \item \texttt{'negative'}: list,
    \item \texttt{'neutral'}: list\},
\end{itemize}

\item \texttt{'word\_counts'}: \{
\begin{itemize}
    \item \texttt{'pos\_words'}: int,
    \item \texttt{'neg\_words'}: int,
    \item \texttt{'total\_words'}: int\},
\end{itemize}

\item \texttt{'absolutisms'}: list (words like 'zawsze', 'nigdy', 'kompletnie'),
\item \texttt{'absolutism\_count'}: int (number of absolutism words),
\item \texttt{'absolutism\_factor'}: float (intensity multiplier, typically 0.5),
\item \texttt{'personal\_pronouns'}: \{
\begin{itemize}
    \item \texttt{'first\_person'}: int,
    \item \texttt{'second\_person'}: int,
    \item \texttt{'third\_person'}: int\},
\end{itemize}
\item \texttt{'type\_token\_ratio'}: float (lexical diversity),
\item \texttt{'repetitions'}: \{
\begin{itemize}
    \item \texttt{'words'}: list,
    \item \texttt{'phrases'}: list,
    \item \texttt{'count'}: int\},
\end{itemize}

\item \texttt{'base\_sentiment'}: float (-1.0 to 1.0, base emotional polarity),
\item \texttt{'intensity\_multiplier'}: float (≥1.0, amplification factor from absolutisms),
\item \texttt{'sentiment\_score'}: float (-1.0 to 1.0, final score after intensity amplification and clamping),
\item \texttt{'sentiment\_components'}: \{
\begin{itemize}
    \item \texttt{'raw\_score'}: float,
    \item \texttt{'clamped\_score'}: float\},
\end{itemize}
\item \texttt{'emotional\_intensity'}: float (0-1, overall emotional intensity),
\item \texttt{'key\_emotional\_phrases'}: list (most emotionally significant phrases),
\item \texttt{'communication\_style'}: str (description of customer's communication pattern)
\end{itemize}
\end{quote}
\end{description}

\subsection{Affective Shift Coefficient}

\begin{description}
\item[Description:]
\begin{quote}
Affective shift coefficient measuring emotional change between turns using formulas: 

$\Delta\texttt{Val} = Valence_t - Valence_{t-1}$

$\Delta\texttt{Aro} = Arousal_t - Arousal_{t-1}$

$\Delta\texttt{Val\_norm} = \Delta Val/\sigma Val$

$\Delta\texttt{Aro\_norm} = \Delta Aro/\sigma Aro$ 

\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'valence\_shift'}: float (change in valence from previous turn), assign 0 if no previous turn,
\item \texttt{'arousal\_shift'}: float (change in arousal from previous turn), assign 0 if no previous turn,
\item \texttt{'valence\_shift\_normalized'}: float (normalized valence change, unbounded), assign 0 if no previous turn,
\item \texttt{'arousal\_shift\_normalized'}: float (normalized arousal change, unbounded), assign 0 if no previous turn,
\item \texttt{'shift\_magnitude'}: float (overall magnitude of emotional change), assign 0 if no previous turn,
\item \texttt{'shift\_direction'}: str (one of: 'improving', 'deteriorating', 'stable'),
\item \texttt{'normalization\_params'}: \{
\begin{itemize}
    \item \texttt{'sigma\_val'}: float,
    \item \texttt{'sigma\_aro'}: float\},
\end{itemize}

\item \texttt{'shift\_interpretation'}: str (explanation of emotional change and its implications),
\item \texttt{'consultant\_response\_needed'}: bool (whether immediate intervention is recommended),
\item \texttt{'recommended\_action'}: str (suggested consultant response to emotional shift)
\end{itemize}
\end{quote}
\end{description}

\subsection{Affective Change Dynamics}

\begin{description}
\item[Description:]
\begin{quote}
Affective change dynamics analyzing emotional trajectory effectiveness using formulas: 

$\texttt{AffectiveTrajectory\_slope} = LinearRegression(Valence\_t, t).slope$

$\texttt{EmotionalStabilization} = StandardDeviation(Arousal\_[t-window:t])$
\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'emotional\_trajectory'}: \{
\begin{itemize}
    \item \texttt{'slope'}: float (linear regression slope),
    \item \texttt{'r\_squared'}: float (fit quality),
    \item \texttt{'trend'}: str\},
\end{itemize}

\item \texttt{'trajectory\_calculation'}: \{
\begin{itemize}
    \item \texttt{'valence\_points'}: list,
\item \texttt{'time\_points'}: list,
\item \texttt{'regression\_equation'}: str\},
\end{itemize}

\item \texttt{'emotional\_stabilization'}: \{
\begin{itemize}
    \item \item \texttt{'arousal\_std'}: float (standard deviation),
    \item \texttt{'stability\_score'}: float (0-1)\},
\end{itemize}

\item \texttt{'stabilization\_window'}: \{
\begin{itemize}
    \item \texttt{'window\_size'}: int,
    \item \texttt{'arousal\_values'}: list\},
\end{itemize}

\item \texttt{'conversation\_effectiveness'}: float (0-1, how well emotional state was managed),
\item \texttt{'emotional\_milestones'}: list (key moments of emotional change),
\item \texttt{'consultant\_performance'}: \{
\begin{itemize}
    \item \texttt{'empathy\_score'}: float,
\item \texttt{'response\_timing'}: str,
\item \texttt{'effectiveness'}: str\},
\end{itemize}

\item \texttt{'overall\_emotional\_arc'}: str (description of entire emotional journey),
\item \texttt{'improvement\_suggestions'}: list (recommendations for better emotional management),
\item \texttt{'emotional\_resolution'}: str (final emotional state assessment)
\end{itemize}
\end{quote}
\end{description}

\section{CognitiveStyleAnalysis}

\subsection{Flesch Kincaid Analysis}

\begin{description}
\item[Description:]
\begin{quote}
FKRS analysis with delta calculations.\par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'current\_fkrs'}: float,
    \item \texttt{'comparison\_fkrs'}: float (from relevant speaker history),
    \item \texttt{'readability\_gap'}: float (absolute difference),
    \item \texttt{'readability\_level'}: str,
    \item\texttt{'adaptation\_needed'}: bool, 
    \item \texttt{'volatility\_score'}: float (for customer turns),
    \item \texttt{'adaptation\_effectiveness'}: float (for consultant turns)
\end{itemize}
     
\end{quote}
\end{description}

\subsection{Sentence Length Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Sentence length analysis: \par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'avg\_sentence\_length'}: float (words per sentence in current turn),
    \item \texttt{'comparison\_avg'}: float (average from speaker's previous turns),
    \item \texttt{'rhythm\_match'}: str (e.g., 'well-matched', 'too\_dense', 'too\_fragmented'),
    \item \texttt{'complexity\_level'}: str (e.g., 'simple', 'moderate', 'complex') 
\end{itemize}

\end{quote}
\end{description}

\subsection{Syntactic Complexity Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Syntactic complexity
\par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'complex\_sentences'}: int (count of complex sentences in current turn),
    \item \texttt{'complexity\_ratio'}: float (complex sentences / total sentences),
    \item \texttt{'comparison\_complexity'}: float (ratio from speaker's previous turns),
    \item \texttt{'match\_level'}: str (e.g., 'well-aligned', 'too\_convoluted', 'overly\_simplistic')
    
\end{itemize}
   
\end{quote}
\end{description}

\subsection{Abstractness Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Abstractness assessment\par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'abstract\_terms'}: int (count of abstract concepts like 'lojalność', 'użyteczność'),
    \item \texttt{'concrete\_terms'}: int (count of concrete objects like 'telefon', 'kabel'),
    \item \texttt{'abstractness\_ratio'}: float (abstract terms / total content words),
    \item \texttt{'communication\_style'}: str (e.g., 'highly\_concrete', 'balanced', 'highly\_abstract')
    
\end{itemize}
   
\end{quote}
\end{description}

\subsection{Technical Terms Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Technical terminology\par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'technical\_count'}: int (count of telecom technical terms),
    \item \texttt{'jargon\_density'}: float (technical terms / total words),
    \item \texttt{'domain\_appropriateness'}: str (e.g., 'well-suited', 'excessive\_jargon', 'too\_simplified'),
    \item \texttt{'customer\_comprehension\_risk'}: str (e.g., 'low\_risk', 'moderate\_risk', 'high\_confusion\_risk')

    
\end{itemize}
,   
\end{quote}
\end{description}

\subsection{Style Adaptation Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Style adaptation assessment with speaker-specific analysis\par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'adaptation\_score'}: float (0-1, how well consultant adapts to customer OR customer consistency), 
    \item \texttt{'cognitive\_alignment'}: str (e.g., 'excellent\_match', 'moderate\_gaps', 'significant\_mismatch'),
    \item  \texttt{'recommendations'}: list (specific adaptation suggestions), 
    \item \texttt{'style\_evolution'}: str (how speaker's style changed over conversation), 
    \item \texttt{'volatility\_analysis'}: (FOR CUSTOMER: \{
    \begin{itemize}
        \item \texttt{'volatility\_score'}: float (0-1), 
        \item \texttt{'style\_changes'}: list,
        \item \texttt{'stability\_assessment'}: str\}), 
    \end{itemize}
     \texttt{'adaptation\_compliance'}: (FOR CONSULTANT: \{
    \begin{itemize}
        \item \texttt{'adaptation\_effectiveness'}: float (0-1)\}),
        \item \texttt{'improvement\_areas'}: list, 
    \end{itemize}
     \texttt{'delta\_calculations'}: \{
     \begin{itemize}
         \item  \texttt{'fkrs\_delta'}: float,
         \item \texttt{'complexity\_delta'}: float,
         \item \texttt{'formality\_delta'}: float\}
     \end{itemize}
    \item 
    
\end{itemize}

\end{quote}
\end{description}

\subsection{Overall Cognitive Fit}

\begin{description}
\item[Description:]
\begin{quote}
Overall cognitive fit assessment\par
\textbf{Dictionary containing:}\par
\begin{itemize}
    \item \texttt{'fit\_score'}: float (0-1, overall cognitive alignment between speakers),
    \item \texttt{'primary\_issues'}: list (main cognitive mismatches identified),
    \item \texttt{'adaptation\_priority'}: str (e.g., 'reduce complexity', 'increase formality', 'maintain current style'),
    \item \texttt{'communication\_effectiveness'}: str (e.g., 'excellent match', 'good alignment', 'significant gaps', 'poor adaptation')
    
\end{itemize}
   
\end{quote}
\end{description}

\section{ConversationEngagementAnalysis}

\subsection{Dialogue Turns Per Time}

\begin{description}
\item[Description:]
\begin{quote}
Dialogue turns per time unit analysis using formula: 

\texttt{LTJC} = (Total Dialogue Turns) / (Session Duration in minutes)

Count all turns from conversation\_history plus current turn. Calculate actual session duration from timestamps. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'total\_turns'}: int (customer turns + consultant turns),
\item \texttt{'user\_turns'}: int (number of customer utterances),
\item \texttt{'system\_turns'}: int (number of consultant responses),
\item \texttt{'session\_duration\_minutes'}: float (total conversation time),
\item \texttt{'session\_duration\_seconds'}: float (total conversation time in seconds),
\item \texttt{'turns\_per\_minute'}: float (calculated LTJC value),
\item \texttt{'conversation\_intensity'}: str (interpretation: 'low', 'moderate', 'high', 'None' in case of no turns),
\item \texttt{'tempo\_assessment'}: str (detailed analysis of conversation pace),
\item \texttt{'engagement\_indicators'}: list (signals of high/low engagement from tempo),
\item \texttt{'recommended\_action'}: str (suggested consultant response to tempo)
\end{itemize}
\end{quote}
\end{description}

\subsection{Average Utterance Length}

\begin{description}
\item[Description:]
\begin{quote}
Average user utterance length analysis using formula: 

$average\_length\_words = total\_words / total\_utterances$

Analyze all user utterances from conversation history. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'total\_words'}: int (sum of all words in user utterances),
\item \texttt{'total\_utterances'}: int (number of user utterances),
\item \texttt{'average\_length\_words'}: float (calculated average words per turn),
\item \texttt{'length\_distribution'}: \{
\begin{itemize}
    \item \texttt{'min'}: int,
    \item \texttt{'max'}: int,
    \item \texttt{'median'}: float,
    \item \texttt{'std'}: float\},
\end{itemize}

\item \texttt{'utterance\_lengths'}: list (word count for each utterance),
\item \texttt{'engagement\_level'}: str (interpretation: 'low', 'moderate', 'high', 'N/A' if unable to classify),
\item \texttt{'communication\_style'}: str (description of user's verbosity),
\item \texttt{'length\_trend'}: str (interpretation over time: 'increasing', 'decreasing', 'stable', 'None' in case of confusion),
\item \texttt{'detailed\_analysis'}: str (interpretation of length patterns),
\item \texttt{'consultant\_guidance'}: str (how to adapt to user's communication style)
\end{itemize}
\end{quote}
\end{description}

\subsection{User Response Time}

\begin{description}
\item[Description:]
\begin{quote}
User response time analysis using formula: 

\texttt{response\_time} = T_{end} - T_{start}

Calculate response times across conversation history. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'current\_response\_time'}: float (seconds for current turn),
\item \texttt{'average\_response\_time'}: float (mean across all turns),
\item \texttt{'response\_time\_distribution'}: \{
\begin{itemize}
    \item \texttt{'min'}: float,
    \item \texttt{'max'}: float,
    \item \texttt{'median'}: float,
    \item \texttt{'std'}: float\},
\end{itemize}

\item \texttt{'response\_times'}: list (all recorded response times),
\item \texttt{'engagement\_assessment'}: str (interpretation: 'highly engaged', 'moderately engaged', 'disengaged'),
\item \texttt{'attention\_indicators'}: list (signals from response timing),
\item \texttt{'outlier\_responses'}: list (unusually fast/slow responses with explanations),
\item \texttt{'trend\_analysis'}: str (response time trends over conversation),
\item \texttt{'recommended\_pacing'}: str (suggested consultant response timing)
\end{itemize}
\end{quote}
\end{description}

\subsection{Conversation Rhythm Changes}

\begin{description}
\item[Description:]
\begin{quote}
Conversation rhythm changes analysis using formula: 

$\texttt{Rhythm\_Change} = (Pace_i - Pace_{i-1}) / \Delta t$

Calculate rhythm changes across all turns in conversation history. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'pace\_measurements'}: list (tempo measurements over time),
\item \texttt{'rhythm\_changes'}: list (calculated acceleration/deceleration values),
\item \texttt{'pace\_statistics'}: \{
\begin{itemize}
    \item \texttt{'mean'}: float,
    \item \texttt{'std'}: float,
    \item \texttt{'min'}: float,
    \item \texttt{'max'}: float\}, 
\end{itemize}

\item \texttt{'acceleration\_points'}: list (moments of significant speedup),
\item \texttt{'deceleration\_points'}: list (moments of significant slowdown),
\item \texttt{'rhythm\_stability'}: float (0-1, measure of tempo consistency),
\item \texttt{'dominant\_rhythm\_pattern'}: str (overall rhythm characterization),
\item \texttt{'emotional\_rhythm\_correlation'}: str (connection between rhythm and emotions),
\item \texttt{'engagement\_rhythm\_analysis'}: str (what rhythm patterns indicate about engagement),
\item \texttt{'consultant\_timing\_recommendations'}: str (how to adapt to rhythm changes)
\end{itemize}
\end{quote}
\end{description}

\section{IntentionAnalysis}

\subsection{Purpose Occurrence}

\begin{description}
\item[Description:]
\begin{quote}
Occurrence of purpose statement using formula: 

\texttt{purpose\_occurrence} = 1 if (intent\_confidence \textgreater{} CT or keyword\_match) else 0, where: 

intent\_confidence: float (0,1)

keyword\_match: True or False based on predefined keywords list (e.g., 'I want to', 'I need') 

CT: Confidence threshold (e.g. 0.85) above which you consider the intent to be detected\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'respond'}: int (0 or 1, calculated using formula)
\item \texttt{'interpretation'}: str (explanation of the decision to label the statement as the intent of the call).
\end{itemize}
\end{quote}
\end{description}

\subsection{Action Intention Convergence}

\begin{description}
\item[Description:]
\begin{quote}
Convergence of actions with intention using formula:

\texttt{convergence} = cos\_sim(embed(intention), embed(action)) \cdot user\_confirmation\_score, where:

cos\_sim(...): Cosine similarity (score -1 to 1) between vectors

embed(intention/action): Vector representations from the language model

user\_confirmation\_score: A multiplier based on the user's response: 1.0 (for 'yes', 'agrees'), -1.0 (for 'no', 'wrong'), 0.5 (neutral/no reaction)\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'convergence'}: float (calculate using formula, if unable to calculate return -1.0)
\item \texttt{'user\_confirmation\_score'}: (calculate based on the description above)
\end{itemize}
\end{quote}
\end{description}F

\subsection{Attempts To Redefine}

\begin{description}
\item[Description:]
\begin{quote}
Number of attempts to redefine the goal using formula: 
\texttt{attempts\_to\_redefine} = count(consultant\_utterance if cls(utterance) == 'clarification\_request')

count(...): Counts the number of occurrences in a given turn 

cls(utterance): Classifier that recognizes the 'request for clarification' type, \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'attempts\_to\_redefine'}: int (calculate using formula)
\item \texttt{'redefine\_list'}: list\textless{}str\textgreater{} (contains attempts to redefine)
\end{itemize}
\end{quote}
\end{description}

\subsection{Response Purpose Cohesion}

\begin{description}
\item[Description:]
\begin{quote}
Consistency of response with purpose using formula: 

\texttt{cohesion} = (w_1*sentiment\_match + w_2*style\_match) * (1 - user\_frustration\_score)

sentiment\_match: 1 - \textbar{}sent(user) - sent(sys)\textbar{}

style\_match: 1 - \textbar{}formal(user) - formal(sys)\textbar{}

user\_frustration\_score: The result (0-1) from the model classifying emotions based on audio features (pitch, jitter, shimmer)\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'cohesion'}: float (calculate using formula)
\item \texttt{'sentiment\_match'}: float (calculate based on the description above)
\item \texttt{'style\_match'}: float (calculate based on the description above)
\item \texttt{'user\_frustration\_score'}: float (calculate based on the description above)
\end{itemize}
\end{quote}
\end{description}

\subsection{Goal Time}

\begin{description}
\item[Description:]
\begin{quote}
Time needed to set a goal using formula: 

\texttt{goal\_time} = turn\_count\_until(Convergence \textgreater{} T\_2)

turn\_count\_until(...): Counts the turns until the convergence metric first exceeds the threshold T\_2,

T\_2: The threshold (e.g. 0.7) above which you consider the goal to have been set, \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'turn\_count\_until'}: int (calculate based on the formula)
\item \texttt{'threshold'}: float (threshold used in formula)
\end{itemize}
\end{quote}
\end{description}

\section{InteractionalEfficiency}

\subsection{Turn Count Efficiency}

\begin{description}
\item[Description:]
\begin{quote}
Turn count to goal achievement. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'turn\_count'}: int (total turns from goal start to completion),
\item \texttt{'benchmark'}: int (task-specific standard),
\item \texttt{'efficiency\_rating'}: str (one of 'excellent', 'good', 'moderate', 'needs improvement', 'poor', 'None' in case of no turns),
\item \texttt{'start\_turn'}: int (turn ID where goal was defined),
\item \texttt{'completion\_turn'}: int (turn ID where goal was completed).
\end{itemize}
\end{quote}
\end{description}

\subsection{Time Efficiency}

\begin{description}
\item[Description:]
\begin{quote}
Time to goal completion. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'total\_time\_seconds'}: float (time from goal start to completion),
\item \texttt{'pause\_time\_seconds'}: float (cumulative silence during interaction),
\item \texttt{'utterance\_time\_seconds'}: float (cumulative speaking time),
\item \texttt{'benchmark\_time'}: float (task-specific standard),
\item \texttt{'delay\_analysis'}: str (e.g., 'long pauses indicate unclear system responses').
\end{itemize}
\end{quote}
\end{description}

\subsection{Repetition Analysis}

\begin{description}
\item[Description:]
\begin{quote}
Repetition/paraphrase count. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'repetition\_count'}: int (number of repeated intents),
\item \texttt{'frustration\_levels'}: list of float (audio frustration scores per repetition, 0-1),
\item \texttt{'repeated\_intents'}: list of str (semantic content of repeated utterances),
\item \texttt{'corrective\_actions'}: list of str (e.g., 'rephrase response', 'ask clarifying question').
\end{itemize}
\end{quote}
\end{description}

\subsection{Response Conciseness}

\begin{description}
\item[Description:]
\begin{quote}
Response conciseness. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'key\_info\_units'}: list of str (extracted entities, values, terms),
\item \texttt{'total\_words'}: int,
\item \texttt{'conciseness\_score'}: float (0-1, key info units / total words),
\item \texttt{'redundancy\_analysis'}: str (e.g., '30\textbackslash{}% of words are non-essential'),
\item \texttt{'compression\_suggestions'}: list of str (e.g., 'use bullet points', 'highlight prices').
\end{itemize}
\end{quote}
\end{description}

\subsection{Off Topic Rate}

\begin{description}
\item[Description:]
\begin{quote}
Off-topic response rate. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'off\_topic\_percentage'}: float (0-100, \textbackslash{}% of off-topic utterances),
\item \texttt{'semantic\_distances'}: list of float (cosine distances from goal vector),
\item \texttt{'off\_topic\_utterances'}: list of str (text of off-topic utterances),
\item \texttt{'redirection\_strategies'}: list of str (e.g., 'gently return to booking', 'confirm goal change').
\end{itemize}
\end{quote}
\end{description}

\subsection{Synthetic Efficiency Score}

\begin{description}
\item[Description:]
\begin{quote}
Synthetic assessment of interaction quality. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'efficiency\_score'}: float (0-1, weighted average of submetrics),
\item \texttt{'strengths'}: list of str (e.g., 'concise responses', 'quick goal completion'),
\item \texttt{'improvement\_priorities'}: list of str (e.g., 'reduce repetitions', 'minimize off-topic digressions'),
\item \texttt{'user\_satisfaction\_inference'}: str (e.g., 'likely satisfied' or 'frustrated due to delays').
\end{itemize}
\end{quote}
\end{description}

\section{PersonalizationAnalysis}

\subsection{Personality Estimate}

\begin{description}
\item[Description:]
\begin{quote}
Estimated customer OCEAN personality traits relevant to service adaptation. This is only for the customer, not the consultant. For the consultant assign -1 for all the traits or N/A for the str fields.\par

\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'traits'}: \{
\begin{itemize}
    \item \texttt{'openness'}: \{
    \begin{itemize}
            \item \texttt{'score'}: float (0-1),
            \item \texttt{'justification'}: str,
            \item \texttt{'confidence'}: float (0-1)\},
    \end{itemize}


    \item \texttt{'conscientiousness'}: \{
    \begin{itemize}
            \item \texttt{'score'}: float (0-1),
            \item \texttt{'justification'}: str,
            \item \texttt{'confidence'}: float (0-1)\},
    \end{itemize}


    \item \texttt{'extraversion'}: \{
    \begin{itemize}
            \item \texttt{'score'}: float (0-1),
            \item \texttt{'justification'}: str,
            \item \texttt{'confidence'}: float (0-1)\},
    \end{itemize}

    \item \texttt{'agreeableness'}: \{
    \begin{itemize}
            \item \texttt{'score'}: float (0-1),
            \item \texttt{'justification'}: str,
            \item \texttt{'confidence'}: float (0-1)\}, 
    \end{itemize}

    \item \texttt{'neuroticism'}: \{
    \begin{itemize}
            \item \texttt{'score'}: float (0-1),
            \item \texttt{'justification'}: str,
            \item \texttt{'confidence'}: float (0-1)\}, \},  
    \end{itemize}

\end{itemize}

\item \texttt{'dominant\_trait'}: str (the most influential trait for this segment),
\item \texttt{'trait\_summary'}: str (high-level interpretation of trait combination for personalization).
\end{itemize}
\end{quote}
\end{description}

\subsection{Adaptation Score}

\begin{description}
\item[Description:]
\begin{quote}
Score and explanation of how well the consultant adapted their communication style to the customer's personality and preferences in this segment. This is only for the consultant, not the customer. For the customer assign -1 for the score and N/A for the str fields.\par

\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'score'}: float (0-1, adaptation effectiveness, -1 for customer turns),
\item \texttt{'adaptation\_type'}: str (e.g., 'mirroring', 'proactive', 'neutral'),
\item \texttt{'explanation'}: str (detailed reasoning for the adaptation score).
\end{itemize}
\end{quote}
\end{description}

\subsection{Personalization Effectiveness}

\begin{description}
\item[Description:]
\begin{quote}
Effectiveness of personalization strategies used in this segment, including use of name, tailored offers, and tone. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'personalized\_elements'}: list (elements used, e.g., ['name', 'offer']),
\item \texttt{'effectiveness\_score'}: float (0-1, overall effectiveness),
\item \texttt{'customer\_reaction'}: str (summary of customer response),
\item \texttt{'suggested\_improvements'}: list (recommendations for future personalization).
\end{itemize}
\end{quote}
\end{description}

\subsection{Customer Engagement Trends}

\begin{description}
\item[Description:]
\begin{quote}
Trends in customer engagement and satisfaction across the call, based on conversation history. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'engagement\_scores'}: list of float (engagement per segment),
\item \texttt{'trend'}: str (e.g., 'increasing', 'stable', 'decreasing'),
\item \texttt{'key\_moments'}: list (segment\_ids or timestamps of notable engagement changes),
\item \texttt{'final\_assessment'}: str (summary of overall engagement and satisfaction).
\end{itemize}
\end{quote}
\end{description}

\section{PredictabilityAndSafetyAnalysis}

\subsection{Risk Keywords Appearance}

\begin{description}
\item[Description:]
\begin{quote}
Risk Keywords Appearance assessment (Metric 1.1) using formula: 

\texttt{risk\_level} = max(Severity(token)) for token in system\_response if token in risk\_dictionaries, \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'risk\_level'}: int (calculated using formula), 'critical\_words\_list: list (identified critical words)
\item \texttt{'risk\_level\_desc'}: str (one of: 'None', 'low', 'medium', 'high/critical')
\item \texttt{'interpretation'}: str (explanation of emotional state and recommended consultant response).
\end{itemize}
\end{quote}
\end{description}

\subsection{Ambigious Answer}

\begin{description}
\item[Description:]
\begin{quote}
Number of ambiguous response ratings (Metric 1.2) using formula: \texttt{ambiguityScore} = Σ Weight(AmbiguousTerm) / Count(TotalSentences), ambiguousTerm: A word or phrase from the ambiguity dictionary (e.g. 'maybe', 'probably', 'could', 'in some cases'). weight(term): The weight assigned to a term, reflecting the degree of ambiguity it introduces (e.g. 'could' \textgreater{} 'sometimes').Sentences: Total number of sentences in the answer\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'ambiguity\_score'}: float (0-1, calculated using formula)
\item \texttt{'ambiguous\_terms'}: list (list of detected terms),
\item \texttt{'interpretation'}: str (explanation of emotional state and recommended consultant response).
\end{itemize}
\end{quote}
\end{description}

\subsection{Answer Entropy}

\begin{description}
\item[Description:]
\begin{quote}
Generative answer entropy using formula: 

$\texttt{response\_entropy} = (1/N) * \Sigma [-\log_{2}(P(token_i))]$, where 

response\_entropy - the average entropy for the entire response

P(token_i): The probability assigned by the model to the selected token i in the given context. High probability (predictable choice) gives a low entropy component, low probability (surprising choice) gives a high entropy component.

N: Total number of tokens in the response,Σ: Sum over all generated tokens.\par

\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'response\_entropy'}: float (0-1, calculated using formula)
\item \texttt{'primary\_topic'}: str (Identified the single, primary topic of the user's implicit or explicit question)
\item \texttt{'off\_topic\_segments'}: list (list of specific sentences or phrases that deviate significantly from the primary topic).
\end{itemize}
\end{quote}
\end{description}

\section{RelationalSynchrony}

\subsection{Formality Level}

\begin{description}
\item[Description:]
\begin{quote}
Formality assessment (Metric 4.1) for the current segment, interpreted according to the speaker's role. If the speaker is 'customer', this measures the customer's formality preference. If the speaker is 'consultant', this measures the consultant's adaptation to the customer's preferred formality. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'formal\_expression\_count'}: int (detected formal phrases),
\item \texttt{'total\_words'}: int,
\item \texttt{'formality\_index'}: float (0–1),
\item \texttt{'is\_formal'}: bool (binary classification),
\item \texttt{'recommended\_consultant\_style'}: str (e.g., 'formal (use Pan/Pani)', 'casual (use ty)'),
\item \texttt{'customer\_style\_interpretation'}: str (e.g., 'Customer prefers formal communication; avoid colloquialisms').
\end{itemize}
\end{quote}
\end{description}

\subsection{Politeness Strategy Metrics}

\begin{description}
\item[Description:]
\begin{quote}
Politeness strategy detection for the current segment, interpreted according to the speaker's role. If the speaker is 'customer', this measures the customer's use of politeness and hedging strategies. If the speaker is 'consultant', this measures the consultant's use of politeness strategies in response to the customer. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'total\_politeness\_strategies'}: int,
\item \texttt{'normalized\_score'}: float,
\item \texttt{'identified\_strategies'}: list,
\item \texttt{'customer\_style\_clue'}: str (e.g., 'Casual tone; consultant may use relatable language'),
\item \texttt{'recommended\_consultant\_tone'}: str (e.g., 'Adopt colloquial phrases to build rapport').
\end{itemize}
\end{quote}
\end{description}

\subsection{Dialogue Convention Usage}

\begin{description}
\item[Description:]
\begin{quote}
Dialogue convention evaluation (Metric 4.3) for the current segment, interpreted according to the speaker's role. If the speaker is 'consultant', this measures the consultant's use of relational conventions (acknowledgments, empathy, clarifying questions). If the speaker is 'customer', this field may be less relevant or used for context. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'total\_conventions\_used'}: int,
\item \texttt{'categorical\_counts'}: \{
\begin{itemize}
    \item \texttt{'acknowledgments'}: int,
    \item \texttt{'empathy'}: int,
    \item \texttt{'clarifying\_questions'}: int\},
\end{itemize}

\item \texttt{'relational\_support\_score'}: float (0–1, \texttt{higher} = better rapport),
\item \texttt{'consultant\_strengths'}: list (e.g., 'Strong use of empathy phrases'),
\item \texttt{'improvement\_opportunities'}: list (e.g., 'Add clarifying questions to validate needs').
\end{itemize}
\end{quote}
\end{description}

\subsection{Metaphor Idiom Usage}

\begin{description}
\item[Description:]
\begin{quote}
Metaphor/idiom detection (Metric 4.4) for the current segment, interpreted according to the speaker's role. If the speaker is 'customer', this measures the customer's use of idioms/metaphors, indicating comfort or informality. If the speaker is 'consultant', this measures the consultant's adaptation to the customer's style using idioms/metaphors. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'total\_idioms\_detected'}: int,
\item \texttt{'normalized\_score'}: float ('total\_idioms\_detected' per 100 words),
\item \texttt{'identified\_expressions'}: list,
\item \texttt{'customer\_style\_clue'}: str (e.g., 'Casual tone; consultant may use relatable language'),
\item \texttt{'recommended\_consultant\_tone'}: str (e.g., 'Adopt colloquial phrases to build rapport').
\end{itemize}
\end{quote}
\end{description}

\subsection{Emotional Tone Synchrony}

\begin{description}
\item[Description:]
\begin{quote}
Emotional synchrony for the current segment, interpreted according to the speaker's role. If the speaker is 'customer', this measures the alignment between the customer's emotional state and the consultant's previous or expected response. If the speaker is 'consultant', this measures how well the consultant's emotional tone matches or adapts to the customer's state. \par
\textbf{Contains:}\par
\begin{itemize}
\item \texttt{'customer\_emotion'}: \{
\begin{itemize}
     \item \texttt{'text'}: str (e.g., 'frustrated'),
\item \texttt{'audio'}: str (e.g., 'high arousal')\},
\end{itemize}

\item \texttt{'consultant\_tone'}: \{
\begin{itemize}
    \item \texttt{'text'}: str (e.g., 'empathic'),
\item \texttt{'audio'}: str (e.g., 'low pitch, slow tempo')\},
\end{itemize}

\item \texttt{'synchrony\_score'}: float (0–1),
\item \texttt{'match\_quality'}: str (e.g., 'high congruence', 'misaligned'),
\item \texttt{'escalation\_risk'}: bool (if score \textless{} 0.3),
\item \texttt{'recommended\_adjustment'}: str (e.g., 'Lower pitch; use phrases like "Przepraszam, że to się stało"').
\end{itemize}
\end{quote}
\end{description}

\section{SemanticAppropriatenessAnalysis}

\subsection{Semantic Similarity}

\begin{description}
\item[Description:]
\begin{quote}
LLM-judged semantic similarity between user question and system answer. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'similarity\_score'}: float (0-1, LLM-judged degree of semantic match),
\item \texttt{'justification'}: str (LLM explanation of why the answer is or is not semantically appropriate),
\item \texttt{'examples\_of\_overlap'}: list (phrases or concepts that match),
\item \texttt{'recommendation'}: str (if low similarity).
\end{itemize}
\end{quote}
\end{description}

\subsection{Keyword Coverage}

\begin{description}
\item[Description:]
\begin{quote}
LLM-judged keyword coverage from question to answer. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'coverage\_score'}: float (0-1, LLM-judged proportion of important question words/concepts present in the answer),
\item \texttt{'question\_keywords'}: list (important words or concepts from question),
\item \texttt{'matched\_keywords'}: list (those found in answer),
\item \texttt{'missing\_keywords'}: list (not found in answer),
\item \texttt{'justification'}: str (LLM explanation of coverage),
\item \texttt{'recommendation'}: str (if coverage is low).
\end{itemize}
\end{quote}
\end{description}

\subsection{Thematic Focus}

\begin{description}
\item[Description:]
\begin{quote}
LLM-judged thematic focus of the answer. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'focus\_score'}: float (0-1, LLM-judged degree to which answer stays on topic),
\item \texttt{'main\_topic'}: str (LLM-identified main topic of the answer),
\item \texttt{'off\_topic\_segments'}: list (phrases or sentences that drift from the topic),
\item \texttt{'justification'}: str (LLM explanation of focus or drift),
\item \texttt{'recommendation'}: str (if focus is low).
\end{itemize}
\end{quote}
\end{description}

\subsection{Logical Consistency}

\begin{description}
\item[Description:]
\begin{quote}
LLM-judged logical consistency and conciseness (Metric 5.4). \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'consistency\_score'}: float (0-1, LLM-judged logical soundness),
\item \texttt{'contradiction\_detected'}: bool (LLM-detected contradiction with question or itself),
\item \texttt{'is\_too\_long'}: bool (LLM-judged excessive length or verbosity),
\item \texttt{'factual\_error\_detected'}: bool (LLM-judged factual error),
\item \texttt{'issues'}: list (LLM-detected problems: contradiction, verbosity, factual error),
\item \texttt{'justification'}: str (LLM explanation),
\item \texttt{'recommendation'}: str (if issues are found).
\end{itemize}
\end{quote}
\end{description}

\subsection{Revision Count}

\begin{description}
\item[Description:]
\begin{quote}
LLM-judged number of system self-corrections/revisions. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'revision\_count'}: int (LLM-detected number of revisions in answer or recent history),
\item \texttt{'revision\_phrases'}: list (phrases indicating revision), 'normalized\_per\_10': float (per 10 answers, if history available),
\item \texttt{'justification'}: str (LLM explanation),
\item \texttt{'recommendation'}: str (if revision count is high).
\end{itemize}
\end{quote}
\end{description}

\subsection{Overall Appropriateness}

\begin{description}
\item[Description:]
\begin{quote}
Overall semantic appropriateness summary. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'appropriateness\_score'}: float (0-1, LLM-judged overall appropriateness),
\item \texttt{'submetric\_scores'}: dict (scores for each sub-metric),
\item \texttt{'final\_assessment'}: str (LLM summary),
\item \texttt{'improvement\_suggestions'}: list (LLM actionable recommendations).
\end{itemize}
\end{quote}
\end{description}

\section{TurnEngagementAnalysis}

\subsection{Current Turn Utterance Length}

\begin{description}
\item[Description:]
\begin{quote}
Current turn utterance length analysis\par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'word\_count'}: int (number of words in current turn),
\item \texttt{'character\_count'}: int (number of characters in current turn),
\item \texttt{'sentence\_count'}: int (number of sentences in current turn),
\item \texttt{'average\_word\_length'}: float (average characters per word),
\item \texttt{'engagement\_level'}: str (interpretation: 'low', 'moderate', 'high', 'N/A' if unable to classify),
\item \texttt{'communication\_style'}: str (description of current turn's verbosity),
\item \texttt{'detailed\_analysis'}: str (interpretation of current turn length),
\item \texttt{'consultant\_guidance'}: str (how to respond to this turn's communication style)
\end{itemize}
\end{quote}
\end{description}

\subsection{Proactive Actions Indicator}

\begin{description}
\item[Description:]
\begin{quote}
Proactive user actions indicator using formula: 

\texttt{WDPU} = (\Sigma Proactive Actions) / (\Sigma Total Relevant Actions) × 100\%. 

CRITICAL LOGIC: If \texttt{speaker} = 'consultant', all proactive action metrics should be 0 (not applicable to consultant), but if \texttt{speaker} = 'customer', analyze current utterance for proactive vs reactive behaviors \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'proactive\_actions'}: list (identified proactive behaviors),
\item \texttt{'reactive\_actions'}: list (identified reactive behaviors),
\item \texttt{'proactive\_count'}: int (number of proactive actions),
\item \texttt{'reactive\_count'}: int (number of reactive actions),
\item \texttt{'total\_actions'}: int (proactive + reactive),
\item \texttt{'proactive\_percentage'}: float (calculated WDPU value),
\item \texttt{'action\_classification'}: \{
\begin{itemize}
    \item \texttt{'questions'}: int,
    \item \texttt{'initiatives'}: int,
    \item \texttt{'explorations'}: int\},
\end{itemize}

\item \texttt{'engagement\_level'}: str (interpretation: 'low', 'moderate', 'high', 'N/A' if unable to classify),
\item \texttt{'user\_initiative\_assessment'}: str (detailed analysis of user initiative),
\item \texttt{'consultant\_response\_strategy'}: str (how to encourage more proactive behavior)
\end{itemize}
\end{quote}
\end{description}

\subsection{Open Ended Questions Presence}

\begin{description}
\item[Description:]
\begin{quote}
Open-ended questions presence analysis using formula: 

\texttt{POPU} = (Open-ended Questions) / (Total Questions) × 100\%. 

LOGIC: Analyze questions in current transcription regardless of speaker. Both customers and consultants can ask questions. \par
\textbf{Dictionary containing:}\par
\begin{itemize}
\item \texttt{'total\_questions'}: int (all questions in current transcription),
\item \texttt{'open\_ended\_questions'}: list (identified open-ended questions),
\item \texttt{'closed\_ended\_questions'}: list (identified closed-ended questions),
\item \texttt{'open\_ended\_count'}: int (number of open-ended questions),
\item \texttt{'closed\_ended\_count'}: int (number of closed-ended questions),
\item \texttt{'open\_ended\_percentage'}: float (calculated POPU value),
\item \texttt{'question\_complexity'}: \{
\begin{itemize}
    \item \texttt{'simple'}: int,
    \item \texttt{'moderate'}: int,
    \item \texttt{'complex'}: int\},
\end{itemize}

\item \texttt{'curiosity\_indicators'}: list (signs of user curiosity and exploration),
\item \texttt{'engagement\_depth'}: str (interpretation of question types),
\item \texttt{'conversation\_development'}: str (how questions drive conversation forward),
\item \texttt{'response\_strategy'}: str (how to handle different question types)
\end{itemize}
\end{quote}
\end{description}

